Parallel Algorithms for Select and Partition with Noisy Comparisons

We consider the problem of finding the $k^{th}$ highest element in a totally ordered set of $n$ elements (select), and partitioning a totally ordered set into the top $k$ and bottom $n-k$ elements (partition) using pairwise comparisons. Motivated by settings like peer grading or crowdsourcing, where multiple rounds of interaction are costly and queried comparisons may be inconsistent with the ground truth, we evaluate algorithms based both on their total runtime and the number of interactive rounds in three comparison models: noiseless (where the comparisons are correct), erasure (where comparisons are erased with probability $1-\gamma$), and noisy (where comparisons are correct with probability $1/2+\gamma/2$ and incorrect otherwise). We provide numerous matching upper and lower bounds in all three models. Even our results in the noiseless model, which is quite well-studied in the TCS literature on parallel algorithms, are novel.

==> adaptive.tex <==
%!TEX root =  Notes.tex

\section{Noiseless, adapative}


%-----------Upper Bound-----------------------------------------------------------------

\subsection{Upper bound}
\subsubsection{2-round}
We provide a 2-round algorithm making $n$ queries in each round.

\begin{enumerate}
\item Round 1:
\begin{enumerate}
\item Pick a random set $S$ of size $s = n^{2/3}$. Pick a random set $K \subset S$ of size $k= n^{1/3}$. (Here we pick $S$ and $K$ with repetition.)
\item Compare every element in $K$ with every element in $S$. 
\item For each element in $K$, we know its ranking among all elements in $S$ from the previous step. Let $x$ be the element in $K$ that is closest to the median of $S$. 
\end{enumerate}
\item Round 2:
\begin{enumerate}
\item Compare every element to $x$. 
\item For each element $i$, if $i$ beats $x$, accept $i$. Otherwise, reject $i$.
\end{enumerate}
\end{enumerate}

\begin{theorem}
\label{thm:2r}
The algorithm above has expected error at most $(1+ \sqrt{2\pi}) n^{2/3}$. 
\end{theorem}
\begin{proof}
We first show that $x$ is close to the median of $S$ by the following lemma.
\begin{lemma}
\label{lem:2r1}
Let $x$'s ranking in $S$ be $p$. Then $\mathbb{E}[|p-s/2|] \leq n^{1/3}$. 
\end{lemma}
\begin{proof}
We know that if $|p-s/2|>i$, it means that there are no elements in $K$ ranks between $s/2 - i$ and $s/2 + i$ in $S$. And the probability that no elements in $K$ ranks between $s/2 - i$ and $s/2 + i$ in $S$ is just $(1- \frac{2i+1}{s})^k$. So we have $Pr[|p-s/2| > i] \leq (1- \frac{2i+1}{s})^k$. Therefore
\[
\mathbb{E}[|p-s/2|]  = \sum_{i=0}^{s/2-1} Pr[|p-s/2| > i] =  \sum_{i=0}^{s/2-1} (1- \frac{2i+1}{s})^k \leq \frac{\sum_{i=0}^{s-1} i^k}{s^k} \leq \frac{\int_0^s i^k di}{s^k} = \frac{s^{k+1}}{(k+1)s^k} < n^{1/3}.
\]
\end{proof}
Then we show $x$ is also close to $n/2$. We need the following lemma.
\begin{lemma}
\label{lem:2r2}
Fix $|p-s/2| = a$, $Pr[|x - n/2| \geq an^{1/3} + i ] \leq  2e^{-\frac{i^2}{2n^{4/3}}}$. 
\end{lemma}
\begin{proof}
Without loss of generality, let's assume $a > 0$. It's easy to see that $Pr[x \geq n/2 + an^{1/3} +i ] \geq Pr[x \leq n/2 - an^{1/3}-i ]$ by symmetry. So we will focus on upper bound $Pr[x \geq n/2 + an^{1/3} +i ]$. Let $X_i$ denote the fraction of elements in $S$ that $n/2 + an^{1/3} + i $ would beat if compared. Notice that $X_i$ is independent with $p$ since $p$ is about rankings inside set $S$ and $X_i$ is about how elements in $S$ are compared with other elements outside $S$. So even when we fix $|p-s/2|$, $X_i$ is the average of $n^{2/3}$ independent random variables and $\mathbb{E}[X_i] = 1/2 + a/n^{2/3}+ i/n$. Therefore, by Chernoff bound, $Pr[X_i \geq 1/2 + a/n^{2/3}] \leq e^{-(i/n)^2 \cdot n^{2/3}/2}$. Thus 
\[
Pr[|x - n/2| \geq an^{1/3} + i ] \leq 2 Pr[x \geq n/2 + an^{1/3} +i ] \leq 2Pr[X_i \geq 1/2 + a/n^{2/3}] \leq 2e^{-\frac{i^2}{2n^{4/3}}}.
\]
\end{proof}
Finally by Lemma \ref{lem:2r1} and Lemma \ref{lem:2r2}, we have 
\begin{eqnarray*}
\E[|x-n/2|] &\leq& \E_p (|p-s/2|\cdot n^{1/3} + \sum_{i=1}^{n/2-|p-s/2|\cdot n^{1/3}} Pr[|x - n/2| \geq |p-s/2| \cdot n^{1/3} + i ]) \\ 
&\leq & \E_p (|p-s/2|\cdot n^{1/3} + \sum_{i=1}^{n/2-|p-s/2|\cdot n^{1/3}}  2e^{-\frac{i^2}{2n^{4/3}}}) \\
&\leq & \E_p (|p-s/2|\cdot n^{1/3} + 2\int_{0}^{+\infty} e^{-\frac{i^2}{2n^{4/3}}} di)\\
&\leq&  \E_p (|p-s/2|\cdot n^{1/3} + \sqrt{\pi \cdot(2n^{4/3})} )\\ 
&\leq& (1+ \sqrt{2\pi}) n^{2/3}.
\end{eqnarray*}
Since our algorithm will only make errors for elements between $x$ and $n/2$. The expected error is at most $\E[|x-n/2|]  = (1+ \sqrt{2\pi}) n^{2/3}$. 
\end{proof}

\input{iter2round}

\subsubsection{4-round}
We provide a 4-round algorithm which has no errors with high probability and makes at most $3n$ queries in each round. It is basically based on the 2-round algorithm and the following observations:
\begin{enumerate}
\item Suppose we know two elements $x_a \leq n/2$ and $x_b \geq n/2$. If we compare them with all other elements, then for every element which is not between $x_a$ and $x_b$, we know whether it is above the median or below the median. 
\item Suppose we have an algorithm $A$ which can find some element between $n/2 - t$ and $n/2 + t$ for all $n$. We can add $2t$ dummy elements which we assume they are always smaller than other elements and run $A$ on $n+2t$ elements. By doing this we will get an element which is between $n/2 - 2t$ and $n/2$ in the original set of elements.  
\end{enumerate}
The 4-round algorithm is the following:
\begin{enumerate}
\item Parameters: Set $\varepsilon$ to be which is at most $1/18$. Set $t = n^{2/3 + \varepsilon}$. 
\item Round 1:
\begin{enumerate}
\item Add $2t$ dummy elements which are smaller than all the other elements. Run the first round of the 2-round algorithm on these $n+2t$ elements. Set $x_a$ be the $x$ returned by the 2-round algorithm. Remove the $2t$ dummy elements.
\item Add $2t$ dummy elements which are larger than all the other elements. Run the first round of the 2-round algorithm on these $n+2t$ elements. Set $x_b$ be the $x$ returned by the 2-round algorithm. Remove the $2t$ dummy elements.
\end{enumerate}
\item Round 2: 
\begin{enumerate}
\item Compare every element to both $x_a$ and $x_b$. 
\item After the previous step, we know the ranking of $x_a$ and $x_b$. If $x_a < n/2 -2t$ or $x_a > n/2$ or $x_b > n/2+2t$ or $x_b < n/2$, then fail. 
\item For each element $i$,
\begin{enumerate}
\item If $i$ beats both $x_a$ and $x_b$, accept $i$. 
\item If both $x_a$ and $x_b$ beat $i$, reject $i$.
\item Otherwise add $i$ to set $U$. 
\end{enumerate}
\item If $|x_a - n/2| < |x_b - n/2|$, add $|x_b - n/2| - |x_a - n/2|$ dummy elements to $U$ which are smaller than all the other elements in $S$.  If $|x_b - n/2| < |x_a - n/2|$, add $|x_a - n/2| - |x_b - n/2|$ dummy elements to $U$ which are larger than all the other elements in $U$. Now the median of $U$ is also $n/2$. 
\end{enumerate}
\item Round 3:
\begin{enumerate}
\item Pick a random set $V \subset U$ of size $v = n /(4t)$. (with repetition)
\item Compare every element in $V$ with every element in $U$. 
\item Now for each element in $V$, we know its ranking in $U$. Let $x_c$ be the largest element in $V$ that is at most $n/2$ and $x_d$ be the smallest element in $V$ that is at least $n/2$. If we cannot find such $x_c$ or $x_d$, then fail. 
\item For each non-dummy element $i$ in $S$,
\begin{enumerate}
\item If $i$ beats both $x_c$ and $x_d$, accept $i$. 
\item If both $x_c$ and $x_d$ beat $i$, reject $i$.
\item Otherwise add $i$ to set $W$. 
\end{enumerate}
\item If $|W| > n^{1/3 + 3\varepsilon}$, then fail. 
\end{enumerate}
\item Round 4:
\begin{enumerate}
\item We know $|W| \leq n^{1/3 + 3\varepsilon} \leq n^{1/2}$. Just compare every two elements in $W$. 
\item We know $n/2$ is in $W$ and which element in $W$ is $n/2$. For each element $i$ in $W$, we just accept or reject $i$ according to the comparison result between $i$ and $n/2$. 
\end{enumerate}
\end{enumerate}


\begin{theorem}
The above algorithm has no errors with probability $1- 2e^{-\frac{n^{\varepsilon}}{2}} - 4e^{-\frac{n^{2\varepsilon}}{32}}-2e^{-\frac{n^{\varepsilon}}{8}}$. 
\end{theorem}
\begin{proof}
Based on the first observation stated before the 4-round algorithm, it is easy to check that if the algorithm does not fail, it has no errors. We only have to upper bound the failure probability. 

To analyze the failure probability in the second round, we need the following lemma which give a high probability bound of 2-round algorithm.
\begin{lemma}
The $x_a$ returned by the first round of the 2-round algorithm satisfied $n/2 - 2t \leq x_a \leq n/2$ with probability at least $1- e^{-\frac{n^{\varepsilon}}{2}} - 2e^{-\frac{n^{2\varepsilon}}{32}}$. 
\end{lemma}
\begin{proof}
The proof is very similar to the proof of Theorem \ref{thm:2r}. One thing to notice is that now we run the first round of the 2-round algorithm on $n+2t$ elements. Let $x$'s ranking in $S$ be $p$. By the same argument as in Lemma \ref{lem:2r1}, $Pr[|p-s/2| > \frac{t}{2(n+2t)^{1/3}}] \leq  (1-\frac{t}{s(n+2k)^{1/3}})^k \leq e^{-\frac{t}{s}}\leq e^{-\frac{n^{\varepsilon}}{2}}$. When $|p-s/2| \leq \frac{t}{2(n+2t)^{1/3}}$, by the same argument as in Lemma \ref{lem:2r2}, $Pr[|x_a - (n/2-t)| > t]  \leq 2e^{-\frac{t^2}{8(n+2t)^{4/3}}} \leq 2e^{-\frac{n^{2\varepsilon}}{32}}$. By Union bound, we know that  with probability at least $1- e^{-\frac{n^{\varepsilon}}{2}} - 2e^{-\frac{n^{2\varepsilon}}{32}}$, $n/2 - 2t \leq x_a \leq n/2$.
\end{proof}
Similarly, with probability at least $1- e^{-\frac{n^{\varepsilon}}{2}} - 2e^{-\frac{n^{2\varepsilon}}{32}}$, $n/2 \leq x_b \leq n/2 +2t$. By Union bound, the probability that the 4-round algorithm failed in the second round is at most $2e^{-\frac{n^{\varepsilon}}{2}} + 4e^{-\frac{n^{2\varepsilon}}{32}}$.

Now let's analyze the failure probability in the third round assuming we succeed in the second round. Let $u$ be the size of $U$. We know $u \leq 4t$. If the followings two conditions were satisfied, we would not fail in the third round.
\begin{enumerate}
\item There is an element in $V$ which ranks between $u/2 - n^{1/3+3\varepsilon}/2$ and $u/2$. 
\item There is an element in $V$ which ranks between $u/2$ and $u/2 + n^{1/3+3\varepsilon}/2$. 
\end{enumerate}
The probability that each condition was not satisfied is at most 
\[
(1-\frac{n^{1/3+3\varepsilon}/2}{u})^v \leq e^{- \frac{n^{1/3+3\varepsilon}/2}{u} \cdot v} \leq e^{-\frac{n^{\varepsilon}}{8}}. 
\]
By Union bound, the failure probability of the third round is at most $2e^{-\frac{n^{\varepsilon}}{8}}$.

To sum up, the 4-round algorithm has no errors with probability at least $1- 2e^{-\frac{n^{\varepsilon}}{2}} - 4e^{-\frac{n^{2\varepsilon}}{32}}-2e^{-\frac{n^{\varepsilon}}{8}}$.
\end{proof}

\subsubsection{3-round}
We provide a 3-round algorithm which has $O(n \log^8 n)$ queries in each round and outputs correctly with high probability. It is simply based on the iterative 2-round algorithm and the intuition in the 4-round algorithm.
\begin{enumerate}
\item Parameters:  Set $t = 256n^{1/2} \log^4 n$. We use iterative 2-round algorithm with parameters same as Corollary \ref{cor:iter2r}. 
\item Round 1:
\begin{enumerate}
\item Add $2t$ dummy elements which are smaller than all the other elements. Run the first round of the iterative 2-round algorithm on these $n+2t$ elements. Set $x_a$ be the $x$ returned by the iterative 2-round algorithm. Remove the $2t$ dummy elements.
\item Add $2t$ dummy elements which are larger than all the other elements. Run the first round of the iterative 2-round algorithm on these $n+2t$ elements. Set $x_b$ be the $x$ returned by the iterative 2-round algorithm. Remove the $2t$ dummy elements.
\end{enumerate}
\item Round 2: 
\begin{enumerate}
\item Compare every element to both $x_a$ and $x_b$. 
\item After the previous step, we know the ranking of $x_a$ and $x_b$. If $x_a < n/2 -2t$ or $x_a > n/2$ or $x_b > n/2+2t$ or $x_b < n/2$, then fail. 
\item For each element $i$,
\begin{enumerate}
\item If $i$ beats both $x_a$ and $x_b$, accept $i$. 
\item If both $x_a$ and $x_b$ beat $i$, reject $i$.
\item Otherwise add $i$ to set $U$. 
\end{enumerate}
\end{enumerate}

\item Round 3:
\begin{enumerate}
\item Compare every two elements in $U$.
\item Now we know which element is the median. Let $x_0$ be the median. 
\item For each element $i \in U$, if $i$ beats $x_0$ accept $i$, otherwise reject $i$.
\end{enumerate}
 
\end{enumerate}
\begin{theorem}
The above algorithm has no errors with probability $1-O(\log n/n^2)$ and has $O(n\log^8 n)$ queries in each round. 
\end{theorem}

\begin{proof}
First it is easy to check that if the algorithm does not fail, it outputs correctly.  In the first round, by Corollary \ref{cor:iter2r}, the algorithm will use at most $2(n+2t)\log (n+2t) = O(n\log n)$ queries. In the second round, the algorithm uses at most $2n$ queries. In the last round, since $U$ has size at most $2t$, so the algorithm will use at most $(2t)^2 = O(n \log^8n)$ queries. Implicitly from the proof of Theorem \ref{thm:iter2r}, we know that with probability $1- O(\log n / n^2)$, $x_a$ is between $n/2-2t$ and $n/2$. Similarly, with probability $1-O(\log n /n^2)$, $x_b$ is between $n/2$ and $n/2+2t$. By Union bound, with probability   $1- O(\log n / n^2)$, we have $x_a$ is between $n/2-2t$ and $n/2$, and $x_b$ is between $n/2$ and $n/2+2t$. So the algorithm fails with probability $1-O(\log n/n^2)$. 
\end{proof}

%-----------Upper Bound-----------------------------------------------------------------

%-----------Lower Bound-----------------------------------------------------------------

\subsection{Lower bound}
\begin{theorem}
\label{thm:2rlb}
Let $d \geq 1$ be some constant. Any 2-round algorithm (maybe randomized) which makes $dn$ queries in each round has error $ \Omega(n^{1/2}/d^{5/2})$ in expectation if the rankings of elements are sampled from uniform distribution. 
\end{theorem}

\begin{proof}
First of all, it is sufficient to prove this theorem for deterministic algorithms. This because the expected error of a randomized algorithm will be the weighted sum of expected error of all the deterministic algorithms it uses. So without the loss of generality, let's assume the 2-round algorithm is a deterministic algorithm.

Suppose the algorithm labels all the elements as $1,...,n$. Let their rankings be $a_1, ... ,a_n$. Then $a_1,...,a_n$ is a uniformly random permutation of $1,...,n$. For any instance of run of the 2-round algorithm, we need to define several terms. Let's pick $S = \{i| n/2-n/(32d) \leq a_i \leq n/2+n/(32d)\}$. Let $s = |S| = n/(16d)$. Let $e(S)$ be the number of queries in the first round whose elements are both in $S$. Then we have 
\[
\E[e(S)] = dn \cdot \frac{n/(16d)}{n} \cdot \frac{n/(16d)-1}{n-1} < n / (256d). 
\]
By averaging argument, with probability at least $3/4$, $e(S) \leq n/(64d)$. Let $A$ be the set of elements that are in $S$ and have not been compared with any other elements in $S$ in the first round of $A$. Then we have $|A| \geq s - 2\cdot e(S)$. If $e(S) \leq n/(64d)$, we have $|A| \geq n/(32d) = s /2$. 

Let's first fix $S$. Then $A$ is fixed by $S$. Let's focus on the case when $|A| \geq s / 2$. Let $A'$ be an arbitrary subset of $A$ of size $s/2$. Let $i_1, ...,i_{s/2}$ be elements in $A'$. Fix the rankings of elements in $\{1,...,n\} - A'$. It's easy to see that $a_{i_1},...,a_{i_{s/2}}$ will be $s/2$ distinct random elements from $n/2 - n/(32d)$ and $n/2 - n/(32d)$. Also, since we have fixed $S$, $A'$ and rankings of elements in $\{1,...,n\}-A'$, the result seen by the algorithm after the first round is fixed. So queries made by the algorithm in the second round is determined. Now let $T = \{i | n/2 - t\sqrt{n}/2 \leq a_i < n/2 + t\sqrt{n}/2\}$. Here $t$ will be determined later. Let $B = A' \cap T$. We have $\E[|B|] = \frac{|T|}{s} \cdot |A'| = t\sqrt{n}/2$. We are going to prove the following claim which we will use to show that in expectation there's constant fraction of elements in $B$ that are not compared with elements in $T$ even after the second round. 
\begin{claim}
Fix $S$, $A'$ and rankings of elements in $\{1,...,n\}-A'$. For each query $(x,y)$ in the second round, the probability that $x \in T$ and $y \in B$ is at most $ \frac{256t^2d^{3/2}}{\sqrt{n}}$. 
\end{claim}
\begin{proof}
We prove this claim by considering two cases.
\begin{enumerate}
\item $x \in A'$: In this case, we have both $x$ and $y$ are in $B$. The probability that this is true is 
\[
\frac{|T|}{s} \cdot \frac{|T|-1|}{s-1} \leq (\frac{|T|}{s})^2 = 256t^2d^2/ n \leq  \frac{256t^2d^{3/2}}{\sqrt{n}}. 
\]
\item $x \in S - A'$: In this case, we need the following lemma:
\begin{lemma}
If we pick $s/2$ random distinct elements from a set $S$ of $s$ elements. Then the $k$-th element of these $s/2$ elements ranked between $s/2 - t\sqrt{n}/2$ and $s/2 + t\sqrt{n}/2$ among $S$ with probability at most $\frac{4t\sqrt{n}}{\sqrt{s}}$. 
\end{lemma}
\begin{proof}
The probability that $k$-th element of these $s/2$ elements ranked between $s/2 - t\sqrt{n}/2$ and $s/2 + t\sqrt{n}/2$ among $S$ is
\[
\sum_{u = s/2 - t\sqrt{n}/2}^{s/2 + t\sqrt{n}/2} \frac{\binom{u-1}{k-1}\binom{s-u}{s/2 - k }}{\binom{s}{s/2}}. 
\]
It is easy to see that $\binom{u-1}{k-1}\binom{s-u}{s/2 - k } \leq \binom{s/2}{s/4}^2$. Therefore, we have 
\[
\sum_{u = s/2 - t\sqrt{n}/2}^{s/2 + t\sqrt{n}/2} \frac{\binom{u-1}{k-1}\binom{s-u}{s/2 - k }}{\binom{s}{s/2}} \leq t\sqrt{n} \cdot \frac{\binom{s/2}{s/4}^2}{\binom{s}{s/2}}. 
\]
By Stirling approximation, we know that $ \sqrt{2\pi} \leq \frac{n!}{n^{n+1/2} e^{-n}} \leq e$. Then we have 
\[
 t\sqrt{n} \cdot \frac{\binom{s/2}{s/4}^2}{\binom{s}{s/2}} \leq  t\sqrt{n} \cdot \frac{e^4}{\sqrt{2\pi}^5} \cdot \frac{\left((s/2)^{s/2} \sqrt{s/2}\right)^4}{\left((s/4)^{s/4}\sqrt{s/4}\right)^4 s^s \sqrt{s}} \leq \frac{4t\sqrt{n}}{\sqrt{s}}. 
\]
\end{proof}
Then we have
\[
Pr[x \in T, y \in B] = Pr[ x \in T] \cdot Pr[y \in B|x \in T] \leq \frac{4t\sqrt{n}}{\sqrt{s}} \cdot \frac{t\sqrt{n}}{s}  = \frac{256t^2d^{3/2}}{\sqrt{n}} .
\]
\end{enumerate}
\end{proof}
Since in the second round, we have $dn$ queries, the expected number of queries that is in the form $(x \in T, y \in B)$ is at most $dn \cdot  \frac{256t^2d^{3/2}}{\sqrt{n}}$. By picking $t = \frac{1}{2048 d^{5/2}}$, we have $dn \cdot  \frac{256t^2d^{3/2}}{\sqrt{n}} \leq t\sqrt{n} /8$ . Let $C \subseteq B$ be the set of elements that have not been compared with other elements in $T$. Then we have $\E[|C|] \geq \E[|B|] - 2 \cdot  (t\sqrt{n} /8) \geq t\sqrt{n}/4$. 

Finally, let's fix the rankings of elements in $A' - C$. Suppose the elements in $C$ are $j_1, ..., j_{|C|}$, then $a_{j_1},...,a_{j_{|C|}}$ are $|C|$ distinct random elements between $n/2 - t\sqrt{n}/2$ and $n/2 + t\sqrt{n}/2$. Also when we fix the rankings of $\{1,...,n\}-C$, the comparison results got by the algorithms in both the first round and the second round are determined. So the output of the algorithm is determined and therefore the algorithm has expected error $|C|/2$. 

To sum up,  any 2-round algorithm (maybe randomized) which makes $dn$ queries in each round has error at least
\[
\frac{3}{4} \cdot (t\sqrt{n}/4) \cdot (1/2) = \Omega(n^{1/2}/d^{5/2}).
\]
\end{proof}
%-----------Lower Bound-----------------------------------------------------------------


==> noisy4rounds.tex <==
%!TEX root =  Notes.tex

\section{Noisy, multiple rounds}

We provide extensions of the noiseless $2$ and $4$-round protocols to settings with noise, incurring an additional factor of $\log n/\epsilon^2$ blow-up. 
\subsection{2-round}
We provide a 2-round algorithm making $n$ queries in each round.

\begin{enumerate}
\item Round 1:
\begin{enumerate}
\item Pick a random set $S$ of size $s = n^{2/3}$. Pick a random set $K \subset S$ of size $k= n^{1/3}$. (Here we pick $S$ and $K$ with repetition.)
\item Compare every element in $K$ with every element in $S$. 
\item For each element in $K$, we know its ranking among all elements in $S$ from the previous step. Let $x$ be the element in $K$ that is closest to the median of $S$. 
\end{enumerate}
\item Round 2:
\begin{enumerate}
\item Compare every element to $x$. 
\item For each element $i$, if $i$ beats $x$, accept $i$. Otherwise, reject $i$.
\end{enumerate}
\end{enumerate}

\begin{theorem}
\label{thm:2r}
The algorithm above has expected error at most $(1+ \sqrt{2\pi}) n^{2/3}$. 
\end{theorem}
\begin{proof}
We first show that $x$ is close to the median of $S$ by the following lemma.
\begin{lemma}
\label{lem:2r1}
Let $x$'s ranking in $S$ be $p$. Then $\mathbb{E}[|p-s/2|] \leq n^{1/3}$. 
\end{lemma}
\begin{proof}
We know that if $|p-s/2|>i$, it means that there are no elements in $K$ ranks between $s/2 - i$ and $s/2 + i$ in $S$. And the probability that no elements in $K$ ranks between $s/2 - i$ and $s/2 + i$ in $S$ is just $(1- \frac{2i+1}{s})^k$. So we have $Pr[|p-s/2| > i] \leq (1- \frac{2i+1}{s})^k$. Therefore
\[
\mathbb{E}[|p-s/2|]  = \sum_{i=0}^{s/2-1} Pr[|p-s/2| > i] =  \sum_{i=0}^{s/2-1} (1- \frac{2i+1}{s})^k \leq \frac{\sum_{i=0}^{s-1} i^k}{s^k} \leq \frac{\int_0^s i^k di}{s^k} = \frac{s^{k+1}}{(k+1)s^k} < n^{1/3}.
\]
\end{proof}
Then we show $x$ is also close to $n/2$. We need the following lemma.
\begin{lemma}
\label{lem:2r2}
Fix $|p-s/2| = a$, $Pr[|x - n/2| \geq an^{1/3} + i ] \leq  2e^{-\frac{i^2}{2n^{4/3}}}$. 
\end{lemma}
\begin{proof}
Without loss of generality, let's assume $a > 0$. It's easy to see that $Pr[x \geq n/2 + an^{1/3} +i ] \geq Pr[x \leq n/2 - an^{1/3}-i ]$ by symmetry. So we will focus on upper bound $Pr[x \geq n/2 + an^{1/3} +i ]$. Let $X_i$ denote the fraction of elements in $S$ that $n/2 + an^{1/3} + i $ would beat if compared. Notice that $X_i$ is independent with $p$ since $p$ is about rankings inside set $S$ and $X_i$ is about how elements in $S$ are compared with other elements outside $S$. So even when we fix $|p-s/2|$, $X_i$ is the average of $n^{2/3}$ independent random variables and $\mathbb{E}[X_i] = 1/2 + a/n^{2/3}+ i/n$. Therefore, by Chernoff bound, $Pr[X_i \geq 1/2 + a/n^{2/3}] \leq e^{-(i/n)^2 \cdot n^{2/3}/2}$. Thus 
\[
Pr[|x - n/2| \geq an^{1/3} + i ] \leq 2 Pr[x \geq n/2 + an^{1/3} +i ] \leq 2Pr[X_i \geq 1/2 + a/n^{2/3}] \leq 2e^{-\frac{i^2}{2n^{4/3}}}.
\]
\end{proof}
Finally by Lemma \ref{lem:2r1} and Lemma \ref{lem:2r2}, we have 
\begin{eqnarray*}
\E[|x-n/2|] &\leq& \E_p (|p-s/2|\cdot n^{1/3} + \sum_{i=1}^{n/2-|p-s/2|\cdot n^{1/3}} Pr[|x - n/2| \geq |p-s/2| \cdot n^{1/3} + i ]) \\ 
&\leq & \E_p (|p-s/2|\cdot n^{1/3} + \sum_{i=1}^{n/2-|p-s/2|\cdot n^{1/3}}  2e^{-\frac{i^2}{2n^{4/3}}}) \\
&\leq & \E_p (|p-s/2|\cdot n^{1/3} + 2\int_{0}^{+\infty} e^{-\frac{i^2}{2n^{4/3}}} di)\\
&\leq&  \E_p (|p-s/2|\cdot n^{1/3} + \sqrt{\pi \cdot(2n^{4/3})} )\\ 
&\leq& (1+ \sqrt{2\pi}) n^{2/3}.
\end{eqnarray*}
Since our algorithm will only make errors for elements between $x$ and $n/2$. The expected error is at most $\E[|x-n/2|]  = (1+ \sqrt{2\pi}) n^{2/3}$. 
\end{proof}

\input{iter2round}

\subsubsection{4-round}
We provide a 4-round algorithm which has no error $\log n / \epsilon^4$ with high probability and makes at most $3n\log n / \epsilon^2$ queries in each round. Note that without resampling, some additive error is necessary. 

The 4-round algorithm is the following:
\begin{enumerate}
\item Parameters: Set $\varepsilon$ to be which is at most $1/18$. Set $t = n^{2/3 + \varepsilon}$. 
\item Round 1:
\begin{enumerate}
\item Add $2t$ dummy elements which are smaller than all the other elements. Run the first round of the 2-round algorithm on these $n+2t$ elements. Set $x_a$ be the $x$ returned by the 2-round algorithm. Remove the $2t$ dummy elements.
\item Add $2t$ dummy elements which are larger than all the other elements. Run the first round of the 2-round algorithm on these $n+2t$ elements. Set $x_b$ be the $x$ returned by the 2-round algorithm. Remove the $2t$ dummy elements.
\end{enumerate}
\item Round 2: 
\begin{enumerate}
\item Compare every element to both $x_a$ and $x_b$. 
\item After the previous step, we know the ranking of $x_a$ and $x_b$. If $x_a < n/2 -2t$ or $x_a > n/2$ or $x_b > n/2+2t$ or $x_b < n/2$, then fail. 
\item For each element $i$,
\begin{enumerate}
\item If $i$ beats both $x_a$ and $x_b$, accept $i$. 
\item If both $x_a$ and $x_b$ beat $i$, reject $i$.
\item Otherwise add $i$ to set $U$. 
\end{enumerate}
\item If $|x_a - n/2| < |x_b - n/2|$, add $|x_b - n/2| - |x_a - n/2|$ dummy elements to $U$ which are smaller than all the other elements in $S$.  If $|x_b - n/2| < |x_a - n/2|$, add $|x_a - n/2| - |x_b - n/2|$ dummy elements to $U$ which are larger than all the other elements in $U$. Now the median of $U$ is also $n/2$. 
\end{enumerate}
\item Round 3:
\begin{enumerate}
\item Pick a random set $V \subset U$ of size $v = n /(4t)$. (with repetition)
\item Compare every element in $V$ with every element in $U$. 
\item Now for each element in $V$, we know its ranking in $U$. Let $x_c$ be the largest element in $V$ that is at most $n/2$ and $x_d$ be the smallest element in $V$ that is at least $n/2$. If we cannot find such $x_c$ or $x_d$, then fail. 
\item For each non-dummy element $i$ in $S$,
\begin{enumerate}
\item If $i$ beats both $x_c$ and $x_d$, accept $i$. 
\item If both $x_c$ and $x_d$ beat $i$, reject $i$.
\item Otherwise add $i$ to set $W$. 
\end{enumerate}
\item If $|W| > n^{1/3 + 3\varepsilon}$, then fail. 
\end{enumerate}
\item Round 4:
\begin{enumerate}
\item We know $|W| \leq n^{1/3 + 3\varepsilon} \leq n^{1/2}$. Just compare every two elements in $W$. 
\item We know $n/2$ is in $W$ and which element in $W$ is $n/2$. For each element $i$ in $W$, we just accept or reject $i$ according to the comparison result between $i$ and $n/2$. 
\end{enumerate}
\end{enumerate}


\begin{theorem}
The above algorithm has no errors with probability $1- 2e^{-\frac{n^{\varepsilon}}{2}} - 4e^{-\frac{n^{2\varepsilon}}{32}}-2e^{-\frac{n^{\varepsilon}}{8}}$. 
\end{theorem}
\begin{proof}
Based on the first observation stated before the 4-round algorithm, it is easy to check that if the algorithm does not fail, it has no errors. We only have to upper bound the failure probability. 

To analyze the failure probability in the second round, we need the following lemma which give a high probability bound of 2-round algorithm.
\begin{lemma}
The $x_a$ returned by the first round of the 2-round algorithm satisfied $n/2 - 2t \leq x_a \leq n/2$ with probability at least $1- e^{-\frac{n^{\varepsilon}}{2}} - 2e^{-\frac{n^{2\varepsilon}}{32}}$. 
\end{lemma}
\begin{proof}
The proof is very similar to the proof of Theorem \ref{thm:2r}. One thing to notice is that now we run the first round of the 2-round algorithm on $n+2t$ elements. Let $x$'s ranking in $S$ be $p$. By the same argument as in Lemma \ref{lem:2r1}, $Pr[|p-s/2| > \frac{t}{2(n+2t)^{1/3}}] \leq  (1-\frac{t}{s(n+2k)^{1/3}})^k \leq e^{-\frac{t}{s}}\leq e^{-\frac{n^{\varepsilon}}{2}}$. When $|p-s/2| \leq \frac{t}{2(n+2t)^{1/3}}$, by the same argument as in Lemma \ref{lem:2r2}, $Pr[|x_a - (n/2-t)| > t]  \leq 2e^{-\frac{t^2}{8(n+2t)^{4/3}}} \leq 2e^{-\frac{n^{2\varepsilon}}{32}}$. By Union bound, we know that  with probability at least $1- e^{-\frac{n^{\varepsilon}}{2}} - 2e^{-\frac{n^{2\varepsilon}}{32}}$, $n/2 - 2t \leq x_a \leq n/2$.
\end{proof}
Similarly, with probability at least $1- e^{-\frac{n^{\varepsilon}}{2}} - 2e^{-\frac{n^{2\varepsilon}}{32}}$, $n/2 \leq x_b \leq n/2 +2t$. By Union bound, the probability that the 4-round algorithm failed in the second round is at most $2e^{-\frac{n^{\varepsilon}}{2}} + 4e^{-\frac{n^{2\varepsilon}}{32}}$.

Now let's analyze the failure probability in the third round assuming we succeed in the second round. Let $u$ be the size of $U$. We know $u \leq 4t$. If the followings two conditions were satisfied, we would not fail in the third round.
\begin{enumerate}
\item There is an element in $V$ which ranks between $u/2 - n^{1/3+3\varepsilon}/2$ and $u/2$. 
\item There is an element in $V$ which ranks between $u/2$ and $u/2 + n^{1/3+3\varepsilon}/2$. 
\end{enumerate}
The probability that each condition was not satisfied is at most 
\[
(1-\frac{n^{1/3+3\varepsilon}/2}{u})^v \leq e^{- \frac{n^{1/3+3\varepsilon}/2}{u} \cdot v} \leq e^{-\frac{n^{\varepsilon}}{8}}. 
\]
By Union bound, the failure probability of the third round is at most $2e^{-\frac{n^{\varepsilon}}{8}}$.

To sum up, the 4-round algorithm has no errors with probability at least $1- 2e^{-\frac{n^{\varepsilon}}{2}} - 4e^{-\frac{n^{2\varepsilon}}{32}}-2e^{-\frac{n^{\varepsilon}}{8}}$.
\end{proof}

\subsubsection{3-round}
We provide a 3-round algorithm which has $O(n \log^8 n)$ queries in each round and outputs correctly with high probability. It is simply based on the iterative 2-round algorithm and the intuition in the 4-round algorithm.
\begin{enumerate}
\item Parameters:  Set $t = 256n^{1/2} \log^4 n$. We use iterative 2-round algorithm with parameters same as Corollary \ref{cor:iter2r}. 
\item Round 1:
\begin{enumerate}
\item Add $2t$ dummy elements which are smaller than all the other elements. Run the first round of the iterative 2-round algorithm on these $n+2t$ elements. Set $x_a$ be the $x$ returned by the iterative 2-round algorithm. Remove the $2t$ dummy elements.
\item Add $2t$ dummy elements which are larger than all the other elements. Run the first round of the iterative 2-round algorithm on these $n+2t$ elements. Set $x_b$ be the $x$ returned by the iterative 2-round algorithm. Remove the $2t$ dummy elements.
\end{enumerate}
\item Round 2: 
\begin{enumerate}
\item Compare every element to both $x_a$ and $x_b$. 
\item After the previous step, we know the ranking of $x_a$ and $x_b$. If $x_a < n/2 -2t$ or $x_a > n/2$ or $x_b > n/2+2t$ or $x_b < n/2$, then fail. 
\item For each element $i$,
\begin{enumerate}
\item If $i$ beats both $x_a$ and $x_b$, accept $i$. 
\item If both $x_a$ and $x_b$ beat $i$, reject $i$.
\item Otherwise add $i$ to set $U$. 
\end{enumerate}
\end{enumerate}

\item Round 3:
\begin{enumerate}
\item Compare every two elements in $U$.
\item Now we know which element is the median. Let $x_0$ be the median. 
\item For each element $i \in U$, if $i$ beats $x_0$ accept $i$, otherwise reject $i$.
\end{enumerate}
 
\end{enumerate}
\begin{theorem}
The above algorithm has no errors with probability $1-O(\log n/n^2)$ and has $O(n\log^8 n)$ queries in each round. 
\end{theorem}

\begin{proof}
First it is easy to check that if the algorithm does not fail, it outputs correctly.  In the first round, by Corollary \ref{cor:iter2r}, the algorithm will use at most $2(n+2t)\log (n+2t) = O(n\log n)$ queries. In the second round, the algorithm uses at most $2n$ queries. In the last round, since $U$ has size at most $2t$, so the algorithm will use at most $(2t)^2 = O(n \log^8n)$ queries. Implicitly from the proof of Theorem \ref{thm:iter2r}, we know that with probability $1- O(\log n / n^2)$, $x_a$ is between $n/2-2t$ and $n/2$. Similarly, with probability $1-O(\log n /n^2)$, $x_b$ is between $n/2$ and $n/2+2t$. By Union bound, with probability   $1- O(\log n / n^2)$, we have $x_a$ is between $n/2-2t$ and $n/2$, and $x_b$ is between $n/2$ and $n/2+2t$. So the algorithm fails with probability $1-O(\log n/n^2)$. 
\end{proof}

%-----------Upper Bound-----------------------------------------------------------------

%-----------Lower Bound-----------------------------------------------------------------

\subsection{Lower bound}
\begin{theorem}
\label{thm:2rlb}
Let $d \geq 1$ be some constant. Any 2-round algorithm (maybe randomized) which makes $dn$ queries in each round has error $ \Omega(n^{1/2}/d^{5/2})$ in expectation if the rankings of elements are sampled from uniform distribution. 
\end{theorem}

\begin{proof}
First of all, it is sufficient to prove this theorem for deterministic algorithms. This because the expected error of a randomized algorithm will be the weighted sum of expected error of all the deterministic algorithms it uses. So without the loss of generality, let's assume the 2-round algorithm is a deterministic algorithm.

Suppose the algorithm labels all the elements as $1,...,n$. Let their rankings be $a_1, ... ,a_n$. Then $a_1,...,a_n$ is a uniformly random permutation of $1,...,n$. For any instance of run of the 2-round algorithm, we need to define several terms. Let's pick $S = \{i| n/2-n/(32d) \leq a_i \leq n/2+n/(32d)\}$. Let $s = |S| = n/(16d)$. Let $e(S)$ be the number of queries in the first round whose elements are both in $S$. Then we have 
\[
\E[e(S)] = dn \cdot \frac{n/(16d)}{n} \cdot \frac{n/(16d)-1}{n-1} < n / (256d). 
\]
By averaging argument, with probability at least $3/4$, $e(S) \leq n/(64d)$. Let $A$ be the set of elements that are in $S$ and have not been compared with any other elements in $S$ in the first round of $A$. Then we have $|A| \geq s - 2\cdot e(S)$. If $e(S) \leq n/(64d)$, we have $|A| \geq n/(32d) = s /2$. 

Let's first fix $S$. Then $A$ is fixed by $S$. Let's focus on the case when $|A| \geq s / 2$. Let $A'$ be an arbitrary subset of $A$ of size $s/2$. Let $i_1, ...,i_{s/2}$ be elements in $A'$. Fix the rankings of elements in $\{1,...,n\} - A'$. It's easy to see that $a_{i_1},...,a_{i_{s/2}}$ will be $s/2$ distinct random elements from $n/2 - n/(32d)$ and $n/2 - n/(32d)$. Also, since we have fixed $S$, $A'$ and rankings of elements in $\{1,...,n\}-A'$, the result seen by the algorithm after the first round is fixed. So queries made by the algorithm in the second round is determined. Now let $T = \{i | n/2 - t\sqrt{n}/2 \leq a_i < n/2 + t\sqrt{n}/2\}$. Here $t$ will be determined later. Let $B = A' \cap T$. We have $\E[|B|] = \frac{|T|}{s} \cdot |A'| = t\sqrt{n}/2$. We are going to prove the following claim which we will use to show that in expectation there's constant fraction of elements in $B$ that are not compared with elements in $T$ even after the second round. 
\begin{claim}
Fix $S$, $A'$ and rankings of elements in $\{1,...,n\}-A'$. For each query $(x,y)$ in the second round, the probability that $x \in T$ and $y \in B$ is at most $ \frac{256t^2d^{3/2}}{\sqrt{n}}$. 
\end{claim}
\begin{proof}
We prove this claim by considering two cases.
\begin{enumerate}
\item $x \in A'$: In this case, we have both $x$ and $y$ are in $B$. The probability that this is true is 
\[
\frac{|T|}{s} \cdot \frac{|T|-1|}{s-1} \leq (\frac{|T|}{s})^2 = 256t^2d^2/ n \leq  \frac{256t^2d^{3/2}}{\sqrt{n}}. 
\]
\item $x \in S - A'$: In this case, we need the following lemma:
\begin{lemma}
If we pick $s/2$ random distinct elements from a set $S$ of $s$ elements. Then the $k$-th element of these $s/2$ elements ranked between $s/2 - t\sqrt{n}/2$ and $s/2 + t\sqrt{n}/2$ among $S$ with probability at most $\frac{4t\sqrt{n}}{\sqrt{s}}$. 
\end{lemma}
\begin{proof}
The probability that $k$-th element of these $s/2$ elements ranked between $s/2 - t\sqrt{n}/2$ and $s/2 + t\sqrt{n}/2$ among $S$ is
\[
\sum_{u = s/2 - t\sqrt{n}/2}^{s/2 + t\sqrt{n}/2} \frac{\binom{u-1}{k-1}\binom{s-u}{s/2 - k }}{\binom{s}{s/2}}. 
\]
It is easy to see that $\binom{u-1}{k-1}\binom{s-u}{s/2 - k } \leq \binom{s/2}{s/4}^2$. Therefore, we have 
\[
\sum_{u = s/2 - t\sqrt{n}/2}^{s/2 + t\sqrt{n}/2} \frac{\binom{u-1}{k-1}\binom{s-u}{s/2 - k }}{\binom{s}{s/2}} \leq t\sqrt{n} \cdot \frac{\binom{s/2}{s/4}^2}{\binom{s}{s/2}}. 
\]
By Stirling approximation, we know that $ \sqrt{2\pi} \leq \frac{n!}{n^{n+1/2} e^{-n}} \leq e$. Then we have 
\[
 t\sqrt{n} \cdot \frac{\binom{s/2}{s/4}^2}{\binom{s}{s/2}} \leq  t\sqrt{n} \cdot \frac{e^4}{\sqrt{2\pi}^5} \cdot \frac{\left((s/2)^{s/2} \sqrt{s/2}\right)^4}{\left((s/4)^{s/4}\sqrt{s/4}\right)^4 s^s \sqrt{s}} \leq \frac{4t\sqrt{n}}{\sqrt{s}}. 
\]
\end{proof}
Then we have
\[
Pr[x \in T, y \in B] = Pr[ x \in T] \cdot Pr[y \in B|x \in T] \leq \frac{4t\sqrt{n}}{\sqrt{s}} \cdot \frac{t\sqrt{n}}{s}  = \frac{256t^2d^{3/2}}{\sqrt{n}} .
\]
\end{enumerate}
\end{proof}
Since in the second round, we have $dn$ queries, the expected number of queries that is in the form $(x \in T, y \in B)$ is at most $dn \cdot  \frac{256t^2d^{3/2}}{\sqrt{n}}$. By picking $t = \frac{1}{2048 d^{5/2}}$, we have $dn \cdot  \frac{256t^2d^{3/2}}{\sqrt{n}} \leq t\sqrt{n} /8$ . Let $C \subseteq B$ be the set of elements that have not been compared with other elements in $T$. Then we have $\E[|C|] \geq \E[|B|] - 2 \cdot  (t\sqrt{n} /8) \geq t\sqrt{n}/4$. 

Finally, let's fix the rankings of elements in $A' - C$. Suppose the elements in $C$ are $j_1, ..., j_{|C|}$, then $a_{j_1},...,a_{j_{|C|}}$ are $|C|$ distinct random elements between $n/2 - t\sqrt{n}/2$ and $n/2 + t\sqrt{n}/2$. Also when we fix the rankings of $\{1,...,n\}-C$, the comparison results got by the algorithms in both the first round and the second round are determined. So the output of the algorithm is determined and therefore the algorithm has expected error $|C|/2$. 

To sum up,  any 2-round algorithm (maybe randomized) which makes $dn$ queries in each round has error at least
\[
\frac{3}{4} \cdot (t\sqrt{n}/4) \cdot (1/2) = \Omega(n^{1/2}/d^{5/2}).
\]
\end{proof}
%-----------Lower Bound-----------------------------------------------------------------

